To believe or not to believe: Validating explanation fidelity for dynamic malware analysis

Converting malware into images followed by vision-based deep learning algorithms has shown superior threat detection efficacy compared with classical machine learning algorithms. When malware are visualized as images, visual-based interpretation schemes can also be applied to extract insights of why individual samples are classified as malicious. In this work, via two case studies of dynamic malware classification, we extend the local interpretable model-agnostic explanation algorithm to explain image-based dynamic malware classification and examine its interpretation fidelity. For both case studies, we first train deep learning models via transfer learning on malware images, demonstrate high classification effectiveness, apply an explanation method on the images, and correlate the results back to the samples to validate whether the algorithmic insights are consistent with security domain expertise. In our first case study, the interpretation framework identifies indirect calls that uniquely characterize the underlying exploit behavior of a malware family. In our second case study, the interpretation framework extracts insightful information such as cryptography-related APIs when applied on images created from API existence, but generate ambiguous interpretation on images created from API sequences and frequencies. Our findings indicate that current image-based interpretation techniques are promising for explaining vision-based malware classification. We continue to develop image-based interpretation schemes specifically for security applications.

==> use_cases.tex <==
\section{Case Studies}
%\subsection{Case Study I: Static malware classification}

\subsection{Case Study I}
Our first case study is concerned with detecting anomalies in dynamic program control-flow traces. 
%In our first case study, we consider a model designed to detect anomalies in dynamic program control-flow traces. 
%We start with a detailed explanation of the underlying problem context and classification model followed by an analysis of the results of our interpretation.
The task is to examine whether the PDF files opened by Adobe Acrobat Reader are malicious or not in a Windows\textsuperscript{\textregistered} system. The source of our control-flow data is Intel Processor Trace\textsuperscript{\textregistered} (Intel PT), which is a hardware feature present in modern Intel\textsuperscript{\textregistered} processors\cite{chen2018henet}. Intel PT\textsuperscript{\textregistered} produces a large volume of data within a short time period. For example, tracing Acrobat Reader for one minute yields over \textit{2 million} indirect control-flow transfers including returns and indirect calls and jumps. It becomes a daunting task for human analysts to examine such high volume of transfers for signs of exploitation. Hence it is desired to employ the automated interpretation framework to extract the explanation. 

We collect 1249 benign and 1314 malicious traces from the \textit{pdfka} malware family, where each trace is collected from the targeted program opening a PDF document. Each trace is then disassembled, yielding a linear sequence of the executed basic blocks. A basic block is defined as a sequence of linear instructions ending with a branch, which can be a return, call, jump, conditional branch and so on. Each basic block is assigned a universally unique integer defined as BBID. A fixed length sliding window is moved over the sequence of BBIDs, and a subsequent long short term memory (LSTM) neural network is tasked with learning and predicting the next BBID for any sub-sequence ending with an indirect control-flow transfer. The intuition behind predicting only indirect transfers is that these are the only places where control-flow hijacking can occur during a program execution. The LSTM model is trained using only normal traces of the target program and then its performance is monitored over unlabeled traces. If an anomaly occurs in the trace, this will cause the model's performance to drop below a defined threshold and the trace will be labeled anomalous.

%To generate dynamic malware images, we use a set of weights  on 874 benign traces. The testing set contains 375 benign traces and 1,314 traces of the \textit{pdfka} malware family. Each malicious trace is of a unique document sample from this family. The traces are fed through the underlying model and a sequence of boolean values is recorded to denote whether each BBID prediction was correct or not. These sequences are then used to train our interpretation model. 
The dynamic malware images are generated from the prediction of the LSTM model on the BBIDs, where the white pixels are correct predictions and black pixels are incorrect predictions. 
On these malware images, we apply deep transfer learning using the pre-trained VGG model\cite{simonyan2014very} on ImageNet, freeze the top layers and add additional two fully connected layers each with dropout to retrain on the dynamic malware images. The training and test split is $0.8:0.2$. We set the number of epochs to be 50 with early stopping criterion if the validation loss does not decrease after 10 epochs. We use the model checkpointed at the 32-th epoch. The classification accuracy on test set on is 100\%. This result demonstrates the effectiveness of vision-based deep transfer learning approach for dynamic malware detection and thus it makes sense to examine what interpretation can be generated using the decision boundaries from this model. %(TO DO: this is needed so we first have effective image-based model and then understand the interpretation)


\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{Figs/Carter-data/04a64deeda580c02e5f48107a5788d4b7d6c32d875fbda481176bafc72bcffd9_plot_explanation_cropped.png}
\caption{\label{fig:pt-malicious} Interpretation for a \textit{pdfka} sample.
White pixels are correct predictions by the underlying model and black incorrect. Green denotes
strong support whereas red is strong contradiction. The green regions shown highlight a suspicious control-flow loop.}
\end{figure}

Next we apply the interpretation framework on the generated images to examine the fidelity of explanation. Figure~\ref{fig:pt-malicious} shows the interpretation of one of the \textit{pdfka} traces. Our model marks several spots within a large streak of incorrect predictions as strongly supporting that this trace belongs to the \textit{pdfka} set. From here we can reverse these chunks of BBIDs to get back to the executed instructions. Upon manual inspection, we discover that at this point in the trace, the program makes one particular indirect call several hundred times in a row. By looking at the relative virtual address, we determine that this activity is happening inside the part of \textit{AcroRd32.dll} that parses TIFF images. The most well known exploit against this part of the program is CVE-2010-0188, which matches several online reports about this family's behavior~\cite{PdfkaReport}. We also manually confirm that this pattern does in fact appear in all the \textit{pdfka} traces and none of the benign traces. To further verify, we also create and trace several benign documents containing normal TIFF images and confirm none of them produce the anomalous pattern. Although Acrobat Reader is closed source, making indisputable verification difficult, we believe our manual analysis strongly supports that our interpretation model successfully identified the subsection of the \textit{pdfka} traces that uniquely characterizes the underlying exploit this family relies on. This case study demonstrates the usefulness of the interpretation method on dynamic malware images.

\subsection{Case Study II}

In our second case study, we evaluate three models designed to classify Windows\textsuperscript{R} Portable Executable (PE) files as either malicious or benign. All three models use dynamic features produced by malware and benign software during execution. %We first describe our dataset and how we extract the features used to train our models. Then we present our findings using our interpretation method for each of our three models.

% These samples were collected from the Georgia Tech Research Institute (GTRI) using their internal malware collection and analysis platform APIARY~\cite{APIARY}.
Our malware dataset is comprised of 13,394 Windows\textsuperscript{R} PE samples. These samples were collected from the Georgia Tech Research Institute (GTRI) using their internal malware collection and analysis platform APIARY~\cite{APIARY}. Using AVClass~\cite{sebastian_avclass:_2016}, our malware dataset is made up of 247 families (demonstrating the diversity of our samples).

Our benign dataset is made up of 5,772 samples and was collected by crawling CNET~\cite{CNET}. Specifically, our samples are a mix of Windows\textsuperscript{R} PE and Windows\textsuperscript{R} Installer (MSI) files under 22 different categories (according to CNET) ranging from Audio to Education to Business-related software.

%To collect the features used for our models, 
We ran all of our samples for 2 minutes using a modified version of Cuckoo~\cite{Cuckoo} version 1.2 in Windows 7 32-bit KVM virtual machines with network and random-access memory (RAM) hardware extensions. We used KVM and hardware extensions to introduce as few artifacts indicative of a malware analysis environment as possible. Malware authors have been known to check for system and network-related artifacts (e.g., registry key values and network timing) which they can use to evade analysis (e.g., by performing innocuous activities or terminating early)~\cite{kolbitsch_power_2011,kirat_barecloud:_2014,dinaburg_ether:_2008,royal_entrapment:_2012}. To improve the quality of our malware dataset, we only include samples which ran for the full 2 minutes without terminating early. We also executed the malware samples with 3 days of them being collected by the organization to improve the chances that the malware would perform malicious activities. Finally, to improve the quality of our benign dataset, we only include samples which did not have more than 2 antivirus companies label them as malicious via VirusTotal~\cite{VirusTotal}. We also use Cuckoo to automatically interact with the benign software (via fake mouse-clicks on its GUI) to cause it to reveal a variety of behaviors.

%\textbf{TODO Li: Please explain how you trained each model mentioned below.}
On each set of the dynamic malware images generated from API existence, sequence and frequencies respectively, we again apply transfer learning via VGG network pre-trained on ImageNet, where we freeze the top layers, add customized two additional fully connected layers and a softmax layer to produce the classification result. The training and validation split is 0.8:0.2. We set the number of epochs to be 50 with early stopping criterion if the validation loss does not decrease after 10 epochs. The classification results on three models are the same within statistically significance with an accuracy at 95\%.

Our first model was trained on Windows Application Programming Interface (API) call~\cite{WindowsAPI} sequences. Training intrusion detection systems (IDS) on system call sequences has been studied in past work~\cite{hofmeyr_intrusion_1998}. While it has been shown to be a weak feature~\cite{wagner_mimicry_2002}, we study it here to determine if our method can tell us that it is a weak feature without relying on domain expertise. We randomly selected 3,353 of our benign samples and 6,629 of our malicious samples to train this model. Although training this model resulted in a training and validation accuracy of 94\%, our interpretation results weren't intuitive. While the model was confident in classifying one the benign samples (Fig~\ref{fig:seq:benign}), it wasn't effective at interpreting why this was the case. As opposed to the Intel PT results, there are large sections which are highlighted as contributing the classification of the sample. The most heavily weighted areas make frequent calls to \textit{FindNextFileW} and \textit{GetProcAddress} (among others), but this isn't indicative of benign \emph{or} malicious behavior. When looking at malicious samples, the results are even more ambiguous. It seems the model memorized at least one of the samples entirely (Fig~\ref{fig:seq:malicious}).

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{Figs/Evan-data/api-sequence/int-benign-9239607a18b9ce4c9116e2b52e6b77e65118d90d6d2d2360ecfbd71724d359de-crop.png}
\caption{\label{fig:seq:benign} Interpretation for a benign sample. Each color represents a unique Windows API call during execution. The large light green areas in the top image denote support for the benign class. The dark red areas in the bottom image contradict the support for the benign class.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{Figs/Evan-data/api-sequence/int-malicious-fd4a58a8328428a1167c827f5de1dea045ed02cb934dbe083ea43f20be53f7d0.png}
\caption{\label{fig:seq:malicious} Interpretation for a malicious sample. Each color represents a unique Windows API call during execution. \textbf{TODO Li: Why is there so much contradiction for the malicious sample but so sign of a confidence?} (Li) Let's use this example as a contradicting case. To Evan, please also provide a sensible case from API-existence. }
\end{figure}

Our second model was trained on Windows API call frequencies. System call frequencies have also been studied in past work~\cite{denning_intrusion-detection_1987}. We randomly selected 2,704 of our benign samples and 7,297 of our malicious samples to train this model. Our interpretation results were similar to those of the API call sequence model. There were quite a few benign \emph{and} malicious samples which got memorized by our model. We did find that one of our malicious sample interpretations focused on cryptography-related API calls. Malware has been known to make use of cryptographic functions for encrypting their command-and-control (C\&C) communications, but this certainly isn't indicative of malicious activity as many legitimate applications use encryption.

Our last model was trained on Windows API call existence. System call existence has not been explored in past work to the best of the authors' knowledge. However, it is intuitive to understand that it too is a weak feature to rely on for malware classification. We randomly selected 2,705 of our benign samples and 7,296 of our malicious samples to train this model. The results were surprisingly the most interesting in terms of their interpretation. The regions highlighted were smaller, but still too ambiguous to glean useful information from them. We did find that one of our malicious sample interpretations focused (again) on cryptography-related API calls as well as HTTP-related calls which (again) is a common way for malware to communicate with their C\&C servers through. But this isn't indicative of anything malicious, as legitimate applications perform similar activity (e.g., Internet browser applications).

%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{Figs/Evan-data/api-frequency/test_train.png}
%\caption{\label{fig:test-train-freq} .}
%\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{Figs/Evan-data/api-existence/train_val.png}
%\caption{\label{fig:test-train-existence} .}
%\end{figure}
